Heavy Traffic Analysis of Multi-Class Bipartite Queueing Systems Under FCFS

This paper examines the performance of multi-class multi-server bipartite queueing systems under a FCFS-ALIS service discipline, where each arriving customer is only compatible with a subset of servers. We analyze the system under conventional heavy-traffic conditions, where the traffic intensity approaches one from below. Building upon the formulation and results of Afeche et al. 2021, we generalize the model by allowing the vector of arrival rates to approach the heavy-traffic limit from an arbitrary direction. We characterize the steady-state waiting times of the various customer classes and demonstrate that a much wider range of waiting time outcomes is achievable. Furthermore, we establish that the matching probabilities, i.e., the probabilities of different customer classes being served by different servers, do not depend on the direction along which the system approaches heavy traffic. We also investigate the design of compatibility between customer classes and servers, finding that a service provider who has complete control over the matching can design a delay-minimizing menu by considering only the limiting arrival rates. When some constraints on the compatibility structure exist, the direction of convergence to heavy-traffic affects which menu minimizes delay. Additionally, we discover that the bipartite matching queueing system exhibits a form of Braess's paradox, where adding more connectivity to an existing system can lead to higher average waiting times, despite the fact that neither customers nor servers act strategically.

==> HeavyTraffic.tex <==
\section{Heavy Traffic Regime}\label{sec:heavytraffic}

In this section, we present the  model that we will use to formally study the question of menu design through heavy-traffic asymptotics. First, in \cref{sec:scaling}, we present the specific heavy traffic scaling of the system primitives. Then, in \cref{sec:equi_HT}, we introduce the notion of a {\em heavy traffic} equilibria, which we use to extend \cref{def:eqprofile} to our heavy traffic regime. In \cref{sec:WatingTimeHT}, we discuss how to calculate steady-state waiting times in heavy traffic and also recap a number of formulas derived in \cite{Afecheetal2019} for this purpose. Finally, in \cref{sec:QPHT} we present a quadratic programming (QP) formulation that we will use to approximate the matching probabilities under the FCFS-ALIS service requirement.  


\subsection{Scaling}\label{sec:scaling} 
We will parametrize our systems by $\epsilon$ and let the bipartite matching system approach heavy traffic as $\eps \downarrow 0$.  Specifically, we assume that there are two vectors $A,a \in \RR_{+}^{|\Theta|}$  satisfying:
\[  \sum_{\theta \in \Theta} A_\theta = \sum_{\theta \in \Theta} a_\theta = |\Gamma|, \]
so that the sequence of arrival rates $\htp{\alpha} = \{ \htp{\alpha_\theta}\}_{\theta \in \Theta}$ satisfies (for $\epsilon$ small enough):
\begin{align}
\label{eq:customer_arrival_rate}
    \htp{\alpha_{\theta}} = A_\theta - a_\theta \epsilon \geq 0\quad \mbox{for all } \theta \in \Theta.
\end{align}
Intuitively, in the heavy-traffic regime, the arrival rates $\htp{\alpha}$ approach the limiting rates $A$ along the direction specified by $a$. It follows that the traffic intensity of the $\eps^{\mbox{\tiny th}}$ system 
\[ \htp{\rho} := \frac{\sum_{\theta} \htp{\alpha_\theta} }{ \mu_1 + \cdots + \mu_m} = \frac{|A| - |a|\, \epsilon}{|\Gamma|} = 1-\epsilon\]
approaches one (i.e., 100\% system utilization) as $\epsilon \downarrow 0$. 


We let $\htp{q}=\{\htp{q_\theta}\}_{\theta \in \Theta}$ denote the strategy profile of all customer types in system indexed by $\epsilon$, where $\htp{q_\theta}=(\htp{q_{\theta 1}}, \ldots, \htp{q_{\theta n}})$ and  $\htp{q_{\theta i}}$ is the probability that type $\theta$ joins service class $i$.  For a given $\epsilon >0$, we let $\htp{\cal M}$ denote the class of admissible menus $M$ that are admissible (in the sense of Definition~\ref{def:admissible}). It is not hard to see that the sets $\htp{\cal M}$ are monotonic in $\epsilon$ and so the limit $\widehat{\cal M}:=\lim_{\epsilon \downarrow 0} \htp{\cal M}$ exists. We will refer to $\widehat{\cal M}$ as the set of {\em admissible menus in heavy traffic}.

Given the sequence of arrival rates, and the strategy profile, the arrival rate into service class $i$ is given by:
\begin{align}
\label{eq:class_arrival_rate}
    \htp{\lambda_i}(\htp{q}) = \sum_{\theta \in \Theta} \htp{\alpha_\theta} \htp{q_{\theta i}}.
\end{align}


The steady-state expected waiting time of service class $i$ and the probability that a customer joining service class $i$ will be served by server $j$ under customers' strategy $\htp{q}$ are denoted by $\htp{W_i}(\htp{q})$ and $\htp{p_{ij}}(\htp{q})$, respectively. Similarly, we let $\htp{\delta}$ denote customers' sensitivity to delay. For non-degenerate solutions, the waiting time $\htp{W_i}(\htp{q})$ will grow out of bound as $\epsilon \downarrow 0$.  For this reason, we assume that $\htp{\delta}$ goes to $0$ as $\epsilon \downarrow 0$ in such a way that the product $\htp{\delta}\,\htp{W_i}(\htp{q})$ converges to a well-defined non-trivial limit. In particular, we will assume that $\htp{\delta}=\delta\,\epsilon$ for some fixed constant $\delta>0$ independent of $\epsilon$\footnote{Alternatively, we could consider a slightly more general scaling of $\htp{\delta}$ that only requires
$\lim_{\epsilon \downarrow 0} {\htp{\delta} \over \epsilon} = \delta.$}. Given this scaling, we find convenient to define the scaled mean waiting time  
\begin{equation}\label{eq:scaledW}
\hts{W_i}(\htp{q})  := \epsilon \cdot \htp{W_i}(\htp{q}),
\end{equation}
which remains bounded in heavy traffic.  Finally, the expected utility of a customer type $\theta$ under consumers' strategy $\htp{q}_\theta$ is given by
$$\htp{U}_{\theta i}(\htp{q})=\sum_{j \in S_i} \htp{p}_{ij}(\htp{q})\,V_{\theta j}-\delta\,\hts{W_i}(\htp{q}).$$
Note that neither the valuations $\{V_{\theta j}\}$ nor the vector of service rates  $\Gamma = (\mu_1, \ldots, \mu_m)^\top$ are scaled and they remain constant independent of $\epsilon$.\vspace{0.3cm}


\subsection{Mean Waiting Time in Heavy Traffic}\label{sec:WatingTimeHT}

To work with heavy traffic equilibria, we need to be able to compute the limiting scaled mean waiting times $\widehat{W}^*$ defined in Definition~\ref{def:heavytrafficeqprofile} for a given pre-limit strategy profile $\hat{q}^* + \epsilon \hat{\phi}^*$. We first give the recipe for deriving these limiting mean waiting times building on the results of \cite{Afecheetal2019} (which in turn build on \cite{AdanWeiss2014}), and state and prove their correctness at the end of the Section. The authors in \cite{Afecheetal2019} find the limiting mean waiting times for a special pre-limit heavy traffic system (that is, a specific direction for approaching heavy traffic). The endogeneity of customer strategies in the present setup necessitates a more general treatment of heavy-traffic matching models. To quickly summarize what is to follow: in heavy-traffic, certain subsets of service classes get \textit{pooled} together so that within a single pool (called a \textit{CRP component}) the waiting times of the service classes evolve together leading to asymptotically equal scaled mean waiting times. Aggregating the service classes based on the pools converts the service menu $M$ into a \textit{directed acyclic graph} with vertex set given by these pools, and it turns out that an enumeration of all the topological orders of this directed acyclic graph is required to obtain the limiting steady-state behavior of the matching model. The structure of the computation and the proofs largely follow \cite{Afecheetal2019} and we refer the reader to their work for additional intuition behind the concepts.

\begin{itemize}[leftmargin=1pt]
    \item[] {\bf Step 1:} {\bf Arrival rates for service classes} \\
    Under the heavy-traffic equilibrium profile $\htp{q}_{\theta i} = \hat{q}^*_{\theta i}+\epsilon \hat{\phi}^*_{\theta i}$ (for $\theta \in \Theta, i \in [n]$), we can express the pre-limit arrival rates into service classes using  \eqref{eq:class_arrival_rate} and \eqref{eq:customer_arrival_rate} as:
\begin{align}
    \label{eq:htp_lambda}
    \htp{\lambda_i} = \sum_{\theta \in \Theta} \htp{\alpha_\theta} \htp{q_{\theta i}} = \sum_{\theta \in \Theta} A_\theta \hat{q}^*_{\theta i} - \epsilon \sum_{\theta \in \Theta} (a_\theta \hat{q}^*_{\theta i} - A_\theta \hat{\phi}^*_{\theta i}) + o(\epsilon) =: \Lambda_i - \epsilon \gamma_i + o(\epsilon). 
\end{align}
    Per our discussion earlier, we assume that all service classes are non-empty: either $\Lambda_i > 0$, or otherwise $\gamma_i < 0$. 
    \item[]{\bf Step 2:} {\bf Decomposing the service classes and servers into Complete Resource Pooling (CRP) components via Residual matching} 
    \begin{itemize}%[leftmargin=1pt]
        \item [{\bf (2a)}] {\sf A Flow problem:} The tuple $(n,m,\Lambda, \Gamma, M)$ defines a flow problem on a bipartite graph $[n] \times [m]$ with edge set given by $M=[m_{ij}]$, flow into (service) node $i$ of $\Lambda_i$, and flow out of (server) node $j$ of $\mu_j$. The flow polytope for the tuple $(n,m,\Lambda, \Gamma, M)$ is given by:
    \[  \hspace{-0.8cm}{\cal F} :=\Big\{f=[f_{ij}] \geq 0: \sum_{i \in [n]} f_{ij} = \mu_j,~~\forall j \in {[m]};~~ \sum_{j \in [m]} f_{ij} = \Lambda_i,~~\forall i \in [n];~~ f_{ij}= 0, ~~\forall (i,j) : m_{ij}=0 \Big\}.\]
        By our assumption that $\htp{q}$ is a heavy-traffic equilibrium, there always exists a solution to the flow problem defined above.
        \item [{\bf (2b)}] {\sf Residual Matching:} Using the flow problem in the previous step, we define a \textit{residual matching} of the menu $M$.
        \begin{dfn}\label{def:residualmatching} {\rm (Residual Matching)} For a given $(n,m,\Lambda, \Gamma,M)$, we define the {\em residual matching} $\breve{M}$, where $\breve{M}=[\breve{m}_{ij}]$ satisfies $\breve{m}_{ij}=1$ if and only if there exists a flow $\tilde{f} \in {\cal F}$ such that $\tilde{f}_{ij} > 0$.
        \end{dfn}    
        Intuitively, for a server class $i$ and server $j$ with $m_{ij}=1$ but $\breve{m}_{ij}=0$, the flow of customers from $i$ to $j$ must vanish in the heavy-traffic limit.
    \item [{\bf (2c)}] {\sf CRP components:} The connected components of the residual matching $\breve{M}$ induce a partition of the service classes and servers into \textit{complete resource pooling} components.
    \begin{dfn}\label{def:CRP}{\rm (CRP Component)} Given the tuple $(n,m,\Lambda, \Gamma, M)$ and the induced residual matching $\breve{M}$, we say that the subset  $\mathbb{C}=(\mathcal{C}, \mathcal{S}) \in 2^{[n]}\times 2^{[m]}$ of service classes and servers forms a CRP component if for any pair of nodes $k_1, k_2 \in \mathcal{C}\cup  \mathcal{S}$ there exists a path between $k_1$ and $k_2$ in $\breve{M}$, and $\mathbb{C}$ is maximal in the sense that the condition is violated for any strict superset of $\mathbb{C}$.
\end{dfn}
Intuitively, the ``well-connectedness'' within a CRP component allows shifting load from one service class to another on short time scales, and in particular under FCFS-ALIS policy to balance the waiting times of the service classes within a component. This crucial fact is what lends tractability in the heavy-traffic regime.\\
We let $K$ denote the number of CRP components induced by the residual matching $\breve{M}$, so that the service classes and servers are partitioned as:
\[ [n] = \mathcal{C}_1 \uplus \mathcal{C}_2 \uplus \cdots \uplus \mathcal{C}_K , \quad [m] = \mathcal{S}_1 \uplus \mathcal{S}_2 \uplus \cdots \uplus \mathcal{S}_K , \]
  with   $\mathbb{C}_k = (\mathcal{C}_k, \mathcal{S}_k)$ denoting the $k^{\text{\tiny th}}$ CRP component. We will use $k(i)$ and $k(j)$ to denote the component that service class $i$, or server $j$ are part of (the use should be clear from context).\\
  Abusing notation, we denote the aggregate arrival and service rates for the CRP components under the heavy-traffic equilibrium as: 
        \begin{align}
        \label{eq:CRP_mu_lambda}
        \forall k \in [K] & \ : \ \htp{\widetilde{\lambda}_k} = \sum_{i \in \Ccal_k} \htp{\lambda_i} =: \widetilde{\Lambda}_k - \epsilon \widetilde{\gamma}_k  + o(\epsilon),\quad \mbox{and} \quad  \widetilde{\mu}_k = \sum_{j \in \Scal_k} \mu_j , 
        \end{align}
        where $\widetilde{\Lambda}_k = \sum_{i \in \Ccal_k} \Lambda_i$, and similarly $\widetilde{\gamma}_k = \sum_{i \in \Ccal_k} \gamma_i$. Note that each CRP component must satisfy $\widetilde{\Lambda}_k = \widetilde{\mu}_k$ so that the slack between demand and capacity within a CRP component in heavy-traffic goes to zero as $ \left(  \widetilde{\mu}_k - \htp{ \widetilde{\lambda}_k}  \right)/\epsilon \to \widetilde{\gamma}_k$. However, the slack $\widetilde{\gamma_k}$ can be negative for some components. \\
        Service classes with $\Lambda_i = 0$ forms a separate CRP component with empty server set. We denote the subset of such CRP components by $\Ical_0$:
        \begin{align}
            \Ical_{0} &= \{ k : \widetilde{\Lambda}_k = 0\}.
        \end{align}
        Let $K' := K - |\Ical_0|$, and we will assume that the CRP components are indexed so that the components in $[K] \setminus \Ical_0$ have indices $1,2, \ldots, K'$.
\end{itemize}
\item[]{\bf Step 3:} {\bf DAG (Directed Acyclic Graph) and Topological orders on CRP components}
\begin{itemize}%[leftmargin=1pt]
    \item [{\bf (3a)}] {\sf DAG:} The menu $M$ and the residual matching $\breve{M}$ uniquely induce a directed acyclic graph (DAG) on the collection of CRP components defined in the previous step.

\begin{dfn}\label{def:DAG}{\rm (DAG)} Given the menu $M=[m_{ij}]$, and the CRP components $\{\mathbb{C}_k=(\mathcal{C}_k, \mathcal{S}_k) \colon k=1,\dots,K\}$ induced by the residual matching $\breve{M}$, we define the DAG $\Dcal = ([K], \Acal)$ associated to $M$ as the directed graph whose nodes correspond to the CRP components, and there is a directed arc $(k_1, k_2) \in \Acal$ from component $\mathbb{C}_{k_1}$ to component $\mathbb{C}_{k_2}$ if and only if there exists a service class $i \in  \mathcal{C}_{k_1}$ and a server $j \in \mathcal{S}_{k_2}$ such that $m_{ij}=1$. We use the notation $k_1 \stackrel{\Dcal}{\rightsquigarrow} k_2$ to denote that there is a directed path $k_1$ to $k_2$ in the DAG $\Dcal$.
\end{dfn}
\cite[Lemma 2]{Afecheetal2019} formally proves that the directed graph defined above is in fact acyclic. The DAG intuitively defines a precedence relation among service classes: Since component $k_1$ with a directed arc to component $k_2$ can ``off-load'' its customers to the servers of component $k_2$, the instantaneous waiting time in component $k_1$ can not exceed that in component $k_2$. This intuition is made precise in the proof of Theorem [FILL IN].
\item [{\bf (3b)}] {\sf Topological Orders:} 
As we mentioned earlier, our computation for the heavy-traffic waiting times build on the work of \cite{AdanWeiss2014}. The crucial component of their analysis is a state-space representation for the FCFS-ALIS matching model which involves ranking the busy servers in order of the waiting time of the customers they are serving. As was proved in \cite{Afecheetal2019}, in heavy-traffic this entails restricting attention to only certain permutations of the CRP components which have asymptotically non-zero probability. The topological orders of the the DAG $\Dcal$ are precisely these permutations. The definition we give next differs slightly from \cite{Afecheetal2019} due to the potential presence of CRP components with $\widetilde{\Lambda}_k=0$.

\begin{dfn}\label{def:topologicalorders}{\em (Topological Orders on CRP Components)} Let $\{\mathbb{C}_1, \mathbb{C}_2,\dots,\mathbb{C}_{K'}\}$ be the CRP components with $\widetilde{\Lambda}_k > 0$. Given the DAG $\Dcal = ([K],\Acal)$, we say that a permutation $\sigma=(\sigma(1),\sigma(2),\dots,\sigma(K'))$ of $[K']$ induces a {\rm topological order} $(\mathbb{C}_{\sigma(1)}, \mathbb{C}_{\sigma(2)},\dots,\mathbb{C}_{\sigma(K')})$ of these CRP components if for every pair $(k_1,k_2) \in [K']$ such that $k_1 \stackrel{\Dcal}{\rightsquigarrow} k_2$, we have $\sigma^{-1}(k_2) < \sigma^{-1}(k_1)$. In other words, sink components of $\Dcal$ precede source components. We let ${\cal T}(\Dcal, K')$ denote the set of all permutations $\sigma$ of $[K']$ that induce a topological order on components $\{\mathbb{C}_1,\ldots,\mathbb{C}_{K'}\}$.

Further, for each $\sigma \in \Tcal(\Dcal, K')$, we partition the CRP components $[K]$ by associating a subset for each $k \in [K']$ as follows:
    \begin{align}
    \label{eq:comps_fn}
        \comps(\sigma, k) := \{\sigma(k)\} \union \{ \kappa \in \Ical_0 : k = \max \{ k' \in [K'] : \  \kappa \stackrel{\Dcal}{\rightsquigarrow} \sigma(k') \} \}.
    \end{align}
    In words, for each index $k$, we associate the CRP component corresponding to $\sigma(k)$ as well as all CRP components $\kappa$ with $\widetilde{\Lambda}_\kappa = 0$ (i.e., server-less components) for which the component $\sigma(k)$ is the last component in the topological order $\sigma$ that is reachable from $\kappa$ via a directed path.
\end{dfn}
    We will use the shorthand $\comps^{-1}(\sigma, k)$ to denote the index $\kappa \in [K']$ such that $k \in \comps(\sigma, \kappa)$.
    
    To highlight the difference with \cite{Afeche2019}, under the heavy-traffic regime considered in \cite{Afeche2019} all CRP components have a non-empty server set $\Scal_j$. This is not necessarily true for all menus and heavy-traffic equilibrium strategy profiles in our setting. This results in service classes which are in a CRP component by themselves. However, these CRP components are special in that they have no incoming arc in the DAG $\Dcal$, and can only have a directed arc to CRP components with non-empty server set. The topological orders $\Tcal(\Dcal,K')$ can thus be thought of as preprocessing $\Dcal$ to remove the server-less CRP components $\{\mathbb{C}_{K'+1},\ldots, \mathbb{C}_K\}$ which are ``hanging off'' $\Dcal$, and finding topogical orders on the remaining components. 
    \end{itemize}
\item[] {\bf Step 4:} {\bf Computing $\widehat{W}^*_i$} \\
\cite[Theorem 1]{Afecheetal2019} implies that the limiting heavy-traffic scaled waiting times for all service menus within a CRP component equalize, and hence the problem reduces to finding a scaled mean waiting time per component. We outline the steps building on the concept of topological orders defined previously.
\begin{itemize}%[leftmargin=1pt]
    \item [{\bf (4a)}] {\sf Unnormalized probabilities for permutations:} Let $\Tcal(\Dcal, K') = (\sigma_1, \ldots, \sigma_T)$ be the collection of topological orders on $\{\mathbb{C}_1, \ldots, \mathbb{C}_{K'}\}$ (the components with $\widetilde{\Lambda}_k > 0$). For a topological order $\sigma_t \in \Tcal(\Dcal, K')$ with the associated function $\comps(\sigma_t, \cdot)$ defined in \eqref{eq:comps_fn}, define the unnormalized probability:
    \begin{align}
    \label{eq:Q_def}
        \mathbb{Q}(\sigma_t) &= \prod_{\kappa \in [K']} \frac{1}{\sum_{\ell=1}^\kappa  \widetilde{\gamma}_{\comps(\sigma_t, \ell)}},
    \end{align}
    where we use the shorthand 
    \[ \widetilde{\gamma}_{\comps(\sigma, \ell)} = \sum_{\kappa \in \comps(\sigma, \ell)} \widetilde{\gamma}_\kappa .\]
    \item [{\bf (4b)}] {\sf Waiting time contribution conditioned on permutation:} For a permutation $\sigma_t \in \Tcal(\Dcal, K')$, for any CRP component $\mathbb{C}_k$, we define the waiting time conditioned on the permutation $\sigma_t$ as:
    \begin{align}
        w_{\sigma_t, k} &= \sum_{ \kappa =  \comps^{-1}(\sigma_t, k)  }^{K'} \frac{1}{\sum_{\ell=1}^\kappa \widetilde{\gamma}_{\comps(\sigma_t, \ell)}} .
    \end{align}
    The following Lemma proves that the expression above is well defined.
    \begin{lem}
    \label{lem:slack_positive}
    Under a heavy-traffic equilibrium strategy profile, for all permutations $\sigma_t \in \Tcal(\Dcal, K')$ of CRP components $\{\mathbb{C}_1,\ldots,\mathbb{C}_{K'}\}$ and for all $\kappa \in [K']$,
    \[  \sum_{\ell = 1}^\kappa \widetilde{\gamma}_{\comps(\sigma_t, \ell)} > 0. \]
    \end{lem}
    \item [{\bf (4c)}] {\sf Steady-state mean waiting time for CRP components:} Finally, for a CRP component $\mathbb{C}_k$, we define the limiting scaled mean waiting time as
    \begin{align}
        \label{eq:CRP_W}
        \widetilde{W}_k &= \sum_{t=1}^T \left({\mathbb{Q}(\sigma_t) \over \mathbb{Q}(\sigma_1)+\mathbb{Q}(\sigma_2)+\cdots+\mathbb{Q}(\sigma_T)}\right)\, w_{\sigma_t, k}.
    \end{align}
\end{itemize}
\end{itemize}

Having described the recipe for computing a steady-state mean waiting time per CRP component, we are ready to state the formal theorem relating them to the limiting scaled mean waiting times, $\widehat{W}^*_i$, for service menus defined in Definition~\ref{def:heavytrafficeqprofile}.

\begin{thm}\label{thm:CRPdelay} For a given admissible service menu $M$ and a heavy-traffic strategy profile $\hat{q}^* + \epsilon \hat{\phi}^*$, let $\breve{M}$ be the residual matching and  $\{\mathbb{C}_1,\dots,\mathbb{C}_{K'}, \mathbb{C}_{K'+1}, \dots, \mathbb{C}_{K} \}$ be the collection of CRP components induced by $\breve{M}$. 
Then, service classes that belong to the same CRP component experience the same scaled steady-state mean waiting time in heavy traffic, and the steady-state mean waiting time of CRP class $\mathbb{C}_k$ is given by \eqref{eq:CRP_W}. That is, if $i_1,i_2 \in \mathbb{C}_k$ then
$$ \widehat{W}^*_{i_1}= \widehat{W}^*_{i_2} = \widetilde{W}_k.$$
\end{thm}
{\sc Proof:} See Appendix~\ref{sec:proof_W}. \hfill $\Box$

































It is worth noticing that according to Theorem~\ref{thm:CRPdelay} the only information that is needed to compute the scaled steady-state mean waiting times in heavy traffic is the aggregated structure of the matching $M$ in terms of CRP components and its DAG  and topological orders  together with the vector of scaled capacity slack $\widetilde{\gamma}=(\widetilde{\gamma}_1,\widetilde{\gamma}_2,\dots,\widetilde{\gamma}_K)$. The more granular information about the specific compatibility structure between service classes and servers or the average arrival rates $\Lambda$ and service capacities $\Gamma$ do not affect the computations of the waiting times.


To illustrate the previous derivation of the scaled steady-state mean waiting time in heavy traffic and provide some additional intuition let us conclude this section with a concrete example.

\subsubsection{Illustrative Example}

 Let us consider a service system with four service classes ($n=4$), four servers ($m=4$) and a fixed matching topology $M$ as depicted in \cref{fig:ExWHT}\footnote{Note that we are not including the arrival rates $\htp{\alpha}=\{\htp{\alpha}_\theta\}_{\theta\in \Theta}$ of customer types or their strategies $\htp{q}=\{\htp{q}_{\theta}\}_{\theta \in \Theta}$ since waiting calculations depend directly on the vector $\htp{\lambda}=\{\htp{\lambda}_i\}_{i\in [n]}$.}, with $0< x < \mu_3$ and $\gamma=\{\gamma_i\}_{i \in [n]} \geq 0$.

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=14cm]{Figures/FigExWHT.pdf}
    \caption[Model Description]{\sf \footnotesize Example with four service classes and four servers.}
     \label{fig:ExWHT}
    \end{center}
\end{figure}

In the figure some of the arcs matching service classes to servers are depicted with a continuous-line arrow while others have a dashed-line arrow. This distinction is based on whether an arc belong to the residual matching $\breve {M}$ or not, that is, based on the limiting flow in the arc as $\epsilon \downarrow 0$. A dashed-line indicates an arc that does not belong to $\breve{M}$, i.e., whose flow must necessarily converge to zero. On the other hand,  solid arcs are those that belong to $\breve{M}$, for which a positive flow exists in the limit as $\epsilon \downarrow 0$. For example, class-1 can only be served by server 1 and  $\htp{\lambda}_1 \uparrow \mu_1$ as $\epsilon \downarrow 0$. Hence, as the system utilization approaches one, we expect  that server 1 will essentially allocate all of its time to serve class-1 customers and  the flows $\htp{f}_{21}$ and $\htp{f}_{31}$ (connecting classes 2 and 3 to server 1) will converge to zero. 

Imagine that we remove the dashed-line arcs. As a result the initial matching $M$ reduces to the residual matching $\breve{M}$ (that includes only the continuous-line arrows) and this residual matching gets partitioned into a collection of independent sub-matching systems, each defined by a connected CRP component. \cref{fig:ExWHT_Residual} shows the three CRP ($K=3$) components for the system in \cref{fig:ExWHT}.
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=12cm]{Figures/FigExWHT_Residual.pdf}
    \caption[Model Description]{\sf \footnotesize Residual matching and CRP components for the system in  \cref{fig:ExWHT}.}
     \label{fig:ExWHT_Residual}
    \end{center}
\end{figure}
Each CRP component $\mathbb{C}_k=({\cal C}_k,{\cal S}_k)$ is defined by a subset of service classes ${\cal C}_k$ and a subset of servers ${\cal S}_k$.  For instance, for the third CRP component $\mathbb{C}_3$ in  \cref{fig:ExWHT_Residual} we have that
${\cal C}_3=\{3,4\}$ and ${\cal S}_4=\{3,4\}$.  

Now that we have identified the CRP components of the system, we can establish a partial order among them in the form of a directed acyclic graph (DAG) connecting them. In this DAG, each node is a CRP component and there is an arc from CRP component $\mathbb{C}_{k_1}$ to CRP component $\mathbb{C}_{k_2}$ if and only if there exists an arc in the original matching topology connecting a service class in ${\cal C}_{k_1}$ to a server in ${\cal S}_{k_2}$. In other words, if there exists a dashed-arc connecting $\mathbb{C}_{k_1}$ to $\mathbb{C}_{k_2}$. The DAG corresponding to our example in \cref{fig:ExWHT,fig:ExWHT_Residual} is depicted on the left panel in \cref{fig:ExWHT_DAG}.

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=10cm]{Figures/FigExWHT_DAG.pdf}
    \caption[Model Description]{\sf \footnotesize Direct acyclic graph (DAG) and topological orders for the system in  \cref{fig:ExWHT}.}
     \label{fig:ExWHT_DAG}
    \end{center}
\end{figure}

The DAG defines a collection of topological orders, which are permutations of the CRP components that are consistent with the partial order induced by the DAG. In our example, there are two topological orders, $T=2$, as shown on the right panel in \cref{fig:ExWHT_DAG}.


Once the DAG and its topological orders are determined, we are ready to compute the limiting  scaled waiting times $\{\widehat{W}_i\}_{i\in[n]}$ by invoking \cref{thm:CRPdelay}. First, we use the fact that all service classes within the same CRP component experience the same scaled waiting time. Thus, in our example, service classes 3 and 4 in \cref{fig:ExWHT} have the same scaled waiting time and  $\widehat{W}_{\mathbb{C}_3}=\widehat{W}_3=\widehat{W}_4$. 

The waiting times of the three CRP components conditional on the topological order being $\sigma_1=(\mathbb{C}_1, \mathbb{C}_2,\mathbb{C}_3)$ are given by
$$w_{\sigma_1, \mathbb{C}_1}={1 \over \tilde{\gamma}_1} + {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2} + {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2+\tilde{\gamma}_3}, \quad w_{\sigma_1, \mathbb{C}_2}= {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2} + {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2+\tilde{\gamma}_3}, \quad w_{\sigma_1, \mathbb{C}_3}=  {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2+\tilde{\gamma}_3}.$$
Similarly, the waiting times conditional on the topological order being  $\sigma_2=(\mathbb{C}_1, \mathbb{C}_3,\mathbb{C}_2)$ are given by
$$w_{\sigma_2, \mathbb{C}_1}={1 \over \tilde{\gamma}_1} + {1 \over \tilde{\gamma}_1+\tilde{\gamma}_3} + {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2+\tilde{\gamma}_3}, \quad w_{\sigma_2, \mathbb{C}_3}= {1 \over \tilde{\gamma}_1+\tilde{\gamma}_3} + {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2+\tilde{\gamma}_3}, \quad w_{\sigma_1, \mathbb{C}_2}=  {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2+\tilde{\gamma}_3}.$$

On the other hand, the unnormalized probabilities are equal to
$$\mathbb{Q}(\sigma_1)={1 \over \tilde{\gamma}_1}\times {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2} \times {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2 + \tilde{\gamma}_3}\qquad \mbox{and}\qquad \mathbb{Q}(\sigma_2)={1 \over \tilde{\gamma}_1} \times {1 \over \tilde{\gamma}_1+\tilde{\gamma}_3} \times {1 \over \tilde{\gamma}_1+\tilde{\gamma}_2+\tilde{\gamma}_3}.$$
After some manipulations, we get that 
$$\widehat{W}_{\mathbb{C}_k}=\left(\tilde{\gamma}_1+\tilde{\gamma}_3 \over 2\,\tilde{\gamma}_1+\tilde{\gamma}_2+\tilde{\gamma}_3\right)\,w_{\sigma_1,\mathbb{C}_k}+\left(\tilde{\gamma}_1+\tilde{\gamma}_2 \over 2\,\tilde{\gamma}_1+\tilde{\gamma}_2+\tilde{\gamma}_3\right)\,w_{\sigma_s,\mathbb{C}_k},\qquad k=1,2,3.$$
To appreciate the subtleties of the dependence between the waiting times and the direction of convergence to heavy traffic, let us compare two numerical examples in \cref{fig:ExWHT_Numeric}.
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=15cm]{Figures/FigExWHT_Numeric.pdf}
    \caption[Model Description]{\sf \footnotesize Numerical examples of the steady-state scaled waiting times.}
     \label{fig:ExWHT_Numeric}
    \end{center}
\end{figure}

Note that the arrival rates in the two system converge to the same limit $\lim_{\epsilon \downarrow 0}\htp{\lambda}=(1,2,3,4)$ and that service capacities are also the same. The only difference in these two system is the direction of convergence to heavy traffic captured by the vector of slacks. For the system on the left, we have $\gamma=(1,3,1,3)$ while for the system on the right we have  $\gamma=(2,2,2,2)$. In both cases, however, the cumulative capacity slack is equal to 8. Despite, all these similarities, the waiting times of the two system are quite different, specially for the first service class. On average, the waiting times on the left panel are about 25\% higher than the average waiting times on the right panel.

\subsection{Matching Probabilities under Heavy Traffic Equilibrium}\label{sec:QPHT}
While the problem of computing waiting times under a FCFS-ALIS service discipline simplifies significantly under heavy traffic conditions, computing the matching probabilities $p_{ij}$ remains computational challenging due to the underlying combinatorial structure of the state-space of the system (see \citealp{AdanWeiss2014}). \cite{CaldenteyKaplanWeiss} and \cite{Afecheetal2019} identify a special class of topologies (including spanning forests and complete and quasi-complete graphs) under which the matching probabilities can be computed efficiently. Specifically, for a given menu $M=[m_{ij}]$ in this class of topologies, the matching probabilities $p_{ij}$ can be computed solving the following quadratic program:
\begin{align}\tag{\bf QP}
\label{eq:QP}  \min_{p }~ & \sum_{i \in [n]} \;\sum_{j \in [m]} {\lambda_i \over \mu_j}\,m_{ij}\, p_{ij}^2  \\ 
\nonumber \mbox{subject to} & \quad \sum_{i \in[n]} \lambda_i\, m_{ij}\,p_{ij}=\mu_j\, \quad \forall j \in [m] , \\ 
\nonumber & \quad \sum_{j \in S_i} m_{ij}\,p_{ij}=1 \quad \forall i \in [m] ,\\
\nonumber & \quad p_{ij} \geq 0 \quad \forall (i,j) \in [n] \times [m] .
\end{align}

In general, however, the \ref{eq:QP} formulation only provides an approximation to the actual FCFS-ALIS  matching probabilities (see \citealp{Afecheetal2019} and \citealp{Fazel-Kaplan2018} for detailed numerical experiments) and, to the best of our knowledge, it is still unknown whether there exists a computationally efficient method to determine the exact matching probabilities for an arbitrary matching topology.

In what follows, we will proceed with our analysis using the QP formulation to compute the matching flows. The following facts about an optimal solution to \eqref{eq:QP} are proven in
\cite{Afecheetal2019}.

\begin{prop}\label{prop:QP_prop} Let $M$ be an admissible menu in heavy traffic, i.e., $M \in  \widehat{\cal M}$. Then,
\begin{enumerate}
\item The quadratic program in \eqref{eq:QP} is feasible and admits a unique optimal solution $p^*(M)$. 
\item A feasible matrix of matching probabilities $p(M)=[p_{ij}(M)]$ is the optimal solution to \eqref{eq:QP} if and only if there exist multipliers $(\omega_j,~j \in [m]) $ for the first set of constraints and  $(\eta_i, ~ i \in[n])$ for the second set of constraints satisfying the KKT first order stationarity conditions:
$$ p^*_{ij}(M) = \max\{ \mu_j \left( \eta_i + \omega_j \right), 0 \}, \quad \forall (i,j): m_{ij} = 1.$$
\end{enumerate}
\end{prop} 

The second property is particularly useful because it allows for a simple encoding of the constraints imposed by the QP formulation\footnote{Which is an approximation for the FCFS-ALIS requirements that we need to impose on $p=[p_{ij}]$.} on the matching probabilities. We will come back to this point in \cref{sec:minwait}.





==> Heavy_traffic_illustration.tex <==




\section{Examples}\label{sec:examples}


{\iffalse
{\bf Example 1: A 2 server system equilibrium \`{a} la Section~\ref{sec:value_maximization}} \\
In this example we show the necessity to characterize the strategies as a sequence with a limit $\Phi_\theta$ and direction $\phi_\theta$, instead of only the limiting values $\Phi_\theta$.

Consider a system with $|\Theta|=2$,  $m=2$ and the following parameters:
\begin{align*}
    \Gamma^\top &= (\mu_1, \mu_2) = (1.5, 1) ,\\
    \htp{\alpha} &= (0.5, 2) - \epsilon \cdot (0, 2.5) ,\\
    V &= \left[ \begin{array}{cc} 1 & 0 \\ v & 2 \end{array} \right] ,
\end{align*}
where $v < 2$. That is, type $1$ customers prefer server 1 ($V_{1,1}=1$, $V_{1,2}=0$), while type $2$ customers prefer server 2 ($V_{2,2}=2$, $V_{2,1} = v<2$). We have kept the parameter $v$ free to show how the equilibrium strategy changes as we change $v$.

Consider the menu where we offer $n=2$ service classes, one per server. That is:
\begin{align*}
    M & = \left[ \begin{array}{cc} 1 & 0 \\ 0 & 1 \end{array} \right].
\end{align*}

Since type 2 customers must split between service class 1 and service class 2, their indifference condition implies $\hts{W}_2 - \hts{W}_1 = 2 - v \geq 0$ in any equilibrium, and therefore type 1 customers strictly prefer service class $1$. Therefore the equilibrium strategies of type 2 and type 1 customers can be characterized as:
\begin{align*}
    \htp{q}_{1,1} & = 1 ,\\
    \htp{q}_{2,1} &= 1/2 + \epsilon u, \\
    \htp{q}_{2,2} &= 1/2 - \epsilon u,
\end{align*}
where we will determine $u$ next.



Going through the steps outlined in the previous section for computing $\hts{W}_i$:
\begin{itemize}
    \item The DAG has $K=2$ components: $\Ccal_1 = \{1\}, \Scal_1 = \{1\}$; $\Ccal_2 = \{2\}, \Scal_2 = \{2\}$ with:
    \begin{align*}
        \widetilde{\mu}_1 = 1.5, \quad \widetilde{\Lambda}_1 = 1.5, \quad \widetilde{\gamma}_1 = \frac{5}{4} - 2 u; \\
        \widetilde{\mu}_2 = 1, \quad \widetilde{\Lambda}_2 = 1, \quad \widetilde{\gamma}_2 = \frac{5}{4} + 2 u. 
    \end{align*}
    However, since the DAG is disconnected, $\Acal = \emptyset$, the analysis for waiting time simplifies considerably. Each service class operates as an independent $M/M/1$ queue.
    \item We get the scaled mean waiting time for the server classes as:
        \begin{align*}
        \hts{W}_1 &=  \frac{1}{\widetilde{\gamma}_1} = \frac{4}{5-8u} \\ \hts{W}_2 &=  \frac{1}{\widetilde{\gamma_2}} = \frac{4}{5+8u}. \\
        \end{align*}
\end{itemize}
    Combining with the indifference condition, we get:
    \[ \hts{W}_2 - \hts{W}_1 = \frac{-64u}{25-64u^2} = 2 - v,  \]
    or,
    \[ u =  \frac{25(2-v)}{64(1-v)} .\]
    
In summary, for the existence of equilibrium in the prelimit of the heavy-traffic scaling, we have to allow for mixed strategies which include both a limiting probability {\it as well as} the direction of approach.

\fi}

{\bf Example 2: Computing waiting time and matching probabilities for empty service classes} \\

Consider a system with 3 servers ($m=3$) with service rates $\Gamma = (1, 1, 1)^\top$, and 4 service classes ($n=4$) with the matching matrix:
\begin{align*}
    M = \begin{bmatrix}
    1 & 0 & 0 \\
    0 & 1 & 0 \\
    0 & 0 & 1 \\
    1 & 1 & 1
    \end{bmatrix}.
\end{align*}

We will specify the type set $\Theta$ and valuation matrix $V$ later, but assume that under the status-quo strategy profile, the arrival rates into the four service classes are:
\begin{align*}
        \htp{\lambda}_1 &= 1 - \gamma_1 \epsilon \\         
        \htp{\lambda}_2 &= 1 - \gamma_2 \epsilon \\         
        \htp{\lambda}_3 &= 1 - \gamma_3 \epsilon \\         
        \htp{\lambda}_4 &= 0
\end{align*}

With the above arrival rates, the asymptotic mean waiting times and matching rates for service classes 1, 2, 3 are given by:

\begin{align*}
    \hts{W_1} & = \frac{1}{\gamma_1} , & \quad  P_{11} = 1; \\ 
    \hts{W_2} & = \frac{1}{\gamma_2} , & \quad  P_{22} = 1; \\ 
    \hts{W_3} & = \frac{1}{\gamma_3} , & \quad  P_{33} = 1.
\end{align*}

To find the asymptotic waiting time $\widehat{W_4}$ as per formula \eqref{eq:W_empty}, we begin with the DAG in Figure~\ref{fig:ex_empty_queue}:

    \begin{figure}[t]
        \centering
        \includegraphics[width=1in]{Figures/ex_empty_queue.pdf}
        \caption{DAG for Example 2}
        \label{fig:ex_empty_queue}
    \end{figure}
    
where component $\mathbb{C}_i$ for $i=1,2,3$ correspond to service class $i$ and server $i$; component $\mathbb{C}_4$ corresponds to service class 4 and has no servers. We have $K'=3$, and $\Tcal(\Dcal, K')$ contains all permutations of $\{1,2,3\}$. For each permutation $\sigma \in \Tcal(\Dcal, K')$, $\comps(\sigma, 1) = \{\sigma(1)\}, \comps(\sigma, 2) = \{\sigma(2)\}, \comps(\sigma, 3) = \{\sigma(3),4\}$. That is, $\comps^{-1}(\sigma, k(4)) = \comps^{-1}(\sigma, 4) = 3 = K'$ for all $\sigma$.
Equation \eqref{eq:W_empty} then gives
    \begin{align*}
    \widehat{W_4} & = \frac{\sum_{\sigma \in \Tcal(\Dcal, K')} \left( \prod_{\kappa \in [K']} \frac{1}{\sum_{\ell=1}^\kappa \widetilde{\gamma}_{\comps(\sigma, \ell)}} \right) \left( \sum_{ \kappa =  \comps^{-1}(\sigma, k(i))  }^{K'} \frac{1}{\sum_{\ell=1}^\kappa \widetilde{\gamma}_{\comps(\sigma, \ell)}} \right)}{\sum_{\sigma \in \Tcal(\Dcal, K')} \left( \prod_{\kappa \in [K']} \frac{1}{\sum_{\ell=1}^\kappa \widetilde{\gamma}_{\comps(\sigma, \ell)}} \right)} \\
    &= \frac{\sum_{\sigma \in \Tcal(\Dcal, K')} \left( \prod_{\kappa \in [K']} \frac{1}{\sum_{\ell=1}^\kappa \widetilde{\gamma}_{\comps(\sigma, \ell)}} \right) \left( \sum_{ \kappa =  K'  }^{K'} \frac{1}{\sum_{\ell=1}^\kappa \widetilde{\gamma}_{\comps(\sigma, \ell)}} \right)}{\sum_{\sigma \in \Tcal(\Dcal, K')} \left( \prod_{\kappa \in [K']} \frac{1}{\sum_{\ell=1}^\kappa \widetilde{\gamma}_{\comps(\sigma, \ell)}} \right)} \\
&=     \frac{1}{\sum_{\ell=1}^{K'} \widetilde{\gamma}_{\comps(\sigma, \ell)}} \\
&= \frac{1}{\widetilde{\gamma}_1 + \widetilde{\gamma}_2  + \widetilde{\gamma}_3 }.
    \end{align*}    

To find $P_{4,j}$: we again begin by pretending $\lambda_4^{(\epsilon, \varepsilon)} = \epsilon \varepsilon$. For $\varepsilon$ small enough (so that $M$ is admissible), we go through the same steps as before to find the matching rates for service class 4:
\begin{enumerate}
    \item The possible topological orders of components $\{1,2,3\}$ are all permutations of these. The normalized asymptotic probability (as $\epsilon \to 0$) of permutation $\sigma$ for $\varepsilon$ small enough is:
    \[ \pi(\sigma) = \frac{1}{\widetilde{\gamma}_{\sigma(1)} } \cdot \frac{1}{\widetilde{\gamma}_{\sigma(1)} +\widetilde{\gamma}_{\sigma(2)}  }
    \cdot \frac{1}{\widetilde{\gamma}_{\sigma(1)} +\widetilde{\gamma}_{\sigma(2)} +\widetilde{\gamma}_{\sigma(3)} - \varepsilon  }
    \]
    \item Conditioning on permutation $\sigma$, say $\sigma = (1,2,3)$, the server that a service class 4 job can match to is $\sigma(3)$. For the case of $\sigma = (1,2,3)$, the probability that the job picked up by server $3$ is of class $4$ is $\frac{\epsilon \varepsilon }{\Lambda_3 - \epsilon\gamma_3 + \epsilon \varepsilon} \sim \frac{\epsilon \varepsilon}{\Lambda_3}$. Therefore, the overall matching rate of server class $4$ to, say, server 3 is:
    \begin{align*} 
    f_{4,3} &= \frac{\pi((1,2,3)) \cdot \mu_3 \cdot \frac{\epsilon \varepsilon}{\Lambda_3} + \pi((2,1,3)) \cdot \mu_3 \cdot \frac{\epsilon \varepsilon}{\Lambda_3} }{\sum_{\sigma \in \Tcal(\Dcal,3)} \pi(\sigma)}  \\
    &= \epsilon \varepsilon \frac{\pi((1,2,3)) + \pi((2,1,3))}{\sum_{\sigma \in \Tcal(\Dcal, 3)} \pi(\sigma)} \\
    &= \epsilon \varepsilon \frac{ \frac{1}{\gamma_1 + \gamma_2} \left( \frac{1}{\gamma_1} + \frac{1}{\gamma_2} \right) }{ 
    \frac{1}{\gamma_1 + \gamma_2} \left( \frac{1}{\gamma_1} + \frac{1}{\gamma_2} \right) 
    + \frac{1}{\gamma_2 + \gamma_3} \left( \frac{1}{\gamma_2} + \frac{1}{\gamma_3} \right) 
    + \frac{1}{\gamma_1 + \gamma_3} \left( \frac{1}{\gamma_1} + \frac{1}{\gamma_3} \right) 
    } \\
    &= \epsilon \varepsilon \frac{ \frac{1}{\gamma_1 \gamma_2}  }{
    \frac{1}{\gamma_1 \gamma_2} 
    + \frac{1}{\gamma_2 \gamma_3} 
    + \frac{1}{\gamma_1 \gamma_3}} \\
    & = \frac{\gamma_3}{ \gamma_1 + \gamma_2 + \gamma_3}
    \end{align*}
    Taking the limit $\varepsilon \to 0$, we get the matching probabilities:
    \[ P_{4,3} = \frac{\gamma_3}{ \gamma_1 + \gamma_2 + \gamma_3}.
    \]
    Similarly, 
    \[ P_{4,1} = \frac{\gamma_1}{ \gamma_1 + \gamma_2 + \gamma_3},
    \]
    \[ P_{4,2} = \frac{\gamma_2}{ \gamma_1 + \gamma_2 + \gamma_3}.
    \]
\end{enumerate}

Now consider the utility of a type $\theta$ customer when joining server class $4$:
\begin{align*}
    U_{\theta,4} &= \sum_{j \in [m]} P_{4,j} V_{\theta,j} - \delta \widehat{W_4} \\
    &= \frac{\gamma_1 V_{\theta,1} +\gamma_2 V_{\theta,2} + \gamma_3 V_{\theta,3} }{ \gamma_1 + \gamma_2 + \gamma_3} - \frac{\delta}{\gamma_1 + \gamma_2 + \gamma_3} \\
    &= \sum_{j=1}^3 \frac{\gamma_j}{\gamma_1 + \gamma_2 + \gamma_3} \left( V_{\theta,j} - \delta \frac{1}{3\gamma_j} \right)
\end{align*}
The utility of joining server class $j \neq 4$ is 
\[ U_{\theta, j} = V_{\theta,j} - \frac{\delta}{\gamma_j}. \]
Therefore, it is possible that if the $V_{\theta,j}$ and $\gamma_j$ are close, then type $\theta$ can improve its utility with an infinitesimal deviation to server class 4. 



==> Preliminaries.tex <==
%!TEX root =main.tex
\setcounter{footnote}{1}

\section{Model Description}\label{sec:ModelDescription}
We assume that there is some exogenously given menu of service classes offered, where a service class is defined by the subset of servers that can serve the class. Such a collection can be expressed by a binary compatibility matrix $M \in \{0,1\}^{n \times m}$, where $n \in \mathbb{N}$ is  the number of service classes that are offered and the entries of $M$ specify which service classes can be served by which servers. That is, server class $i$ can be served by server $j$ if and only if $m_{ij}=1$ for $i\in [n]$ and $j\in [m]$. For each service class $i \in [n]$, we let $S_i(M) \subseteq [m]$ denote the subset of servers serving class $i$ under menu $M$. 

Upon arrival, customers select a service class and join the queue of this class and wait to be served according to a FIFO queueing discipline. Servers, on the other hand, have exponential service times and serve the different classes using a FCFS service discipline. We will use $\Gamma = (\mu_1, \ldots, \mu_m)^\top$ to denote the column vector of service rates. We also assume that an arriving customer who finds an empty queue will be routed to the compatible server that has been idle the longest. Under these conditions, we say that the queueuing system operates under a FCFS-ALIS (first come first served - assign longest idle server) service discipline.

To illustrate, Figure~\ref{fig:Ex1} depicts an example with four servers ($m=4$), three service classes ($n=3$) and three customer types ($|\Theta|=3$). 
\begin{figure}[hbt]
    \begin{center}
    \includegraphics[width=10cm]{Figures/Fig_Ex1.pdf}
    \caption[Model Description]{\sf \footnotesize Example with three customer types, three service classes and four servers.}
     \label{fig:Ex1}
    \end{center}
\end{figure}

In this example, the menu $M$ is given by
\begin{equation}
M=\left[\begin{array}{cccc} 1 & 1 & 0 & 1 \\ 1 & 0 & 1 & 1 \\ 0 & 1 & 0 & 1 \end{array}\right],
\end{equation}
that is, class 1 is compatible with servers 1, 2 and 4; class 2 is compatible with servers 1, 3 and 4; and class 3 is compatible with servers 2 and 4. Also, under the FCFS-ALIS service discipline,  if server 2 becomes idle then it will serve the customer from class 1 or class 3 that has been waiting the longest. 


{\sc Waiting Times, Matching Probabilities and Stability}: A strategy profile $q \in \cal{Q}$ induces a vector of arrival rates $\lambda(q)=\{\lambda_i(q)\}_{i \in [n]}$ to each service class, where
\begin{equation*}
\lambda_i(q)=\sum_{\theta \in \Theta}  \alpha_\theta\,q_{\theta i}\qquad i=1,\dots,n.
\end{equation*}
Indirectly, through the vector of arrival rates $\lambda(q)$, the strategy profile $q$ also determines the vector $W(q)=\{W_i(q)\}_{i \in [n]}$ of steady-state waiting times for each class as well as the matrix of matching probabilities $p(q)=(p_{ij}(q)\colon i \in [n], j \in [m])$ between service classes and servers, where $p_{ij}(q)$ denotes the steady-state probability that a customer joining class $i$ will be served by server $j$ under the strategy profile $q$. 

We will restrict our attention to menus $M$ and strategies $q$ that are stable in the sense that they jointly admit a well-defined steady state for the service system. To guarantee the existence of such a steady state, we need to impose a stability requirement on the primitives of the model and the matching topology. The following result was proved in \cite{AdanWeiss2014}.

\begin{prop}\label{prop:stability}{\rm \citep[Theorem 2.1]{AdanWeiss2014}}
The menu $M$ and strategy $q$  admit a steady state 
under a FCFS-ALIS service discipline if and only if the following   condition is satisfied:
\begin{equation*}
\quad \sum_{j \in \mathscr{S}} \mu_j > \sum_{i \in U_{\mathscr{S}}(M)} \lambda_i(q)\qquad \mbox{for all } \mathscr{S} \subseteq [m],
\end{equation*}
where 
\begin{equation*}
U_{\mathscr{S}}(M):= \Big\{i \in [n]\colon \sum_{j \in \mathscr{S}^c} m_{ij}=0\Big\}
\end{equation*}

is the subset of service classes that can only be served by servers in $\mathscr{S}$.
\end{prop}


We will further restrict attention to  {\em admissible} menus $M$ for which the stability condition above is satisfied for some feasible strategy profile $q$. 

\begin{dfn}\label{def:admissible}{\rm (Admissible Menus and Strategies)}  A menu $M$ is {\rm admissible} if there exists a strategy profile $q=\{q_\theta\}_{ \theta \in \Theta}$ for which  the service system is stable, that is, the inequalities in Proposition~\ref{prop:stability} are satisfied.
We let ${\cal M}$ denote the set of admissible menus.

For an admissible menu $M \in {\cal M}$, we denote by ${\cal Q}(M) \subseteq {\cal Q}$ the set of all feasible strategy profiles for which the service system is stable.
\end{dfn}

A necessary and sufficient condition for ${\cal M}$ to be non-empty is that the cumulative arrival rate is strictly less than the cumulative service capacity, $
|\alpha| <|\mu|$. Indeed, under this condition it is not hard to see that any menu $M$ in which every server is connected to at least one service class is admissible. In particular, the single-line menu (i.e., $n=1$ and $m_{1j}=1$ for all $j \in [m]$)  is admissible. 

\vspace{0.3cm}

{\sc Degenerate Equilibria}: One technicality to be aware of in dealing with these systems is that for some systems, an equilibrium may have one or more service classes that no customers join. This requires the calculation of waiting times and matching probabilities for service classes with arrival rates of zero. We can do this by taking the limit of the expected waiting times and matching probabilities as the relevant service class arrival rates converge to zero. We will see an example of this in the following section. 

%\varun{Do we want to comment on this in the heavy-traffic section? The reader may worry that we have a class with $\hat{q}^*_{\theta i} = 0$ but $\hat{\phi}^*_{\theta i} > 0$. So in the pre-limit we always get $\htp{\lambda}_i > 0$ but in the limit it is 0.}
\subsection{Steady state results for fixed arrival rates}\label{sec:adanweissresult}
As our results heavily rely on the steady state analysis of \cite{AdanWeiss2014}, we will briefly review the Markov chain representation the authors use. The authors derive their result based on a Markov chain defined on a novel state space $X$. A state in this state space is described by three components: {\it (i)} a permutation of servers $s = (s_1, \ldots, s_m)$, {\it (ii)} an integer $b \in \{0,\ldots, m\}$ indicating the number of busy servers, and {\it (iii)} a vector $(n_1, \ldots, n_b)$ that indicates the composition of customers waiting for service in the different service classes. It is helpful to denote a generic state $x \in X$ by the tuple:
\[  x = (s_1, n_1, s_2, n_2, \ldots, s_b, n_b, s_{b+1}, \ldots , s_m).\]

The first $b$ components $(s_1,\dots,s_b)$ of the server permutation $s$ denote the $b$ busy servers ranked according to the arrival time of the customer they are serving, with server $s_1$ serving  the oldest arrival and server $s_b$ serving the youngest arrival. The remaining servers $(s_{b+1}, \ldots, s_m)$ are all idle and ranked in the order they became idle, with $s_{b+1}$ the server that has been idle the longest. Finally, $n_\ell$ for $\ell=1,\dots,b$, represents the number of customers in the system who arrived after the job currently being served by $s_{\ell}$ and who can only be served by some server in $(s_1,\dots,s_{\ell})$. That is, each of these $n_\ell$ customers must belong to some service menu in $U( s_1,\ldots, s_\ell )$.

According to \cite[Theorem 2.1]{AdanWeiss2014}, the steady-state probability of state $x$ admits the product form:
\begin{align}\label{eq:steadystate}
\pi(x) &= {\cal B}  \prod_{\ell=1}^b \frac{\lambda^{n_\ell}_{U(s_1,\ldots, s_\ell)} }{\mu_{\{s_1,\ldots, s_\ell\}}^{n_\ell+1} } \prod_{\ell=b+1}^m \lambda_{C(s_\ell, \ldots, s_m)}^{-1},
\end{align}
with ${\cal B}$ an appropriate normalizing constant. Additionally, each of the $n_\ell$ customers `between' server $s_\ell$ and server $s_{\ell+1}$ belongs to service class $i \in U(s_1,\ldots, s_\ell)$ independently with probability $\frac{\lambda_i}{\lambda_{U(s_1,\ldots, s_\ell)}}$.


\subsection{Roadmap of Analysis and Results}

Before moving into the analysis of the decision maker's problem, let us provide a summary of the methodology that we have used to tackle the problem of designing an optimal menu of service classes and the type of results that we have been able to obtain.

One of the major challenges associated to the service provider's optimization problem in \eqref{eq:DM_problem} is the underlying combinatorial structure of the steady-state distribution of the system, which makes it difficult to calculate waiting times and matching rates.  According to \cite{AdanWeiss2014} and based on our own numerical experiments,  the  computation of this steady-state distribution is restricted to relatively small instances with $\max\{n,m\} \leq 12$. To circumvent this challenge we will study the problem under (conventional) heavy traffic conditions, that is, in the limit as the traffic intensity of the system approaches one from below. In \cref{sec:heavytraffic}, we laid out the details of this heavy traffic regime and show how to compute mean waiting times and matching probabilities.

\cref{sec:2server} is devoted to the problem of designing an optimal service menu for the special case in which there are only two servers ($m=2$). The purpose of this section is to highlight some key features of the problem in a setting in which we can provide a complete characterization of an optimal menu as a function of the model’s parameters. In particular, the solution of the two-server case reveals that the different possible service menus can be partitioned into two main groups: (a) menus that achieve the minimum possible average waiting time and (b) menus that achieve the maximum possible average matching reward. Intuitively, delay-minimizing menus are those that are able to induce {\em complete capacity pooling} while reward-maximizing menus are those able to implement the matching that a central planner would select if she had complete control over the assignment of customers to servers. Interesting, with two servers, every admissible service menu follows in one of these two categories.  The solution also shows that out of the set of delay-minimizing menus the single-line produces the lowest possible average matching reward while out of the reward-maximizing menus the dedicated menu (i.e., one service class per server) generates the longest waiting-time delays. In other words, these two simple and commonly used menus  are complete opposite designs when it comes to balancing the trade-off between average matching reward and mean customers' delays and they are both Pareto dominated by other service menus with more complex matching topologies. The single-line is dominated by a menu that achieves strictly higher average reward while preserving {\em complete capacity pooling}. On the other hand, a dedicated menu is dominated by another menu that results from {\em chaining} the dedicated service classes.


In \cref{sec:general_m}, we extend the results of the two-server case to the general case of an arbitrary number of servers. First, we show that the special characteristics of the single-line and dedicated menus that we observe in the two-server setting extend to the case of an arbitrary number of servers. That is, a dedicated menu maximizes the average matching reward (but not necessarily the waiting time delay) (\cref{thm:maxV}) and a single-line menu minimizes both average waiting-time delay and matching reward (\cref{thm:SL_Reward}). Second, we extend the design principles of {\em complete capacity pooling} and {\em chaining}, to identify Pareto optimal menus that achieve the highest possible matching reward among all delay-minimizing menus and menus that achieve the minimum possible delay among reward-maximizing menus. 






adding service classes to a given menu does not necessarily improve the performance of the resulting equilibrium. In addition, it shows 
that the single-line and dedicated menus are complete opposite designs when it comes to balancing the trade-off between average matching reward and mean customers' delays. While the single-line menu minimizes waiting times and minimizes average rewards, the dedicated menu (i.e., one service class per server) achieves exactly the opposite performance. The analysis of the two-server case also reveals that both  single-line and dedicated menus are Pareto dominated by other menus. 



 











==> discussion_old.tex <==
\section{Discussion}\label{sec:discussion}
Before getting into the proofs of our main results, we discuss some of their implications. while highlighting the differences between the behaviours of our model and the model in \cite{Afecheetal2019}. We also explore some simple questions regarding the design of menus of service classes. 

\subsection{Average waits}
We will now turn our attention to the average delays across all service classes in heavy traffic. Similarly to our definition of $ w_{\sigma_t, k}$, for a permutation $\sigma_t \in \Tcal(\Dcal, K')$, we let $\bar{w}_{\sigma_t}$ be the average delay over all service classes conditioned on the permutation $\sigma_t$. The expression for $\bar{w}_{\sigma_t}$ is given by 
\begin{align}
\bar{w}_{\sigma_t} & = \sum_{k = 1}^{K'} \frac{\mu_{\sigma(k)}}{|\mu|}w_{\sigma_t, k}\nonumber \\
& = \sum_{k = 1}^{K'} \frac{\mu_{\sigma(k)}}{|\mu|}\sum_{ \kappa =  \comps^{-1}(\sigma_t, k)  }^{K'} \frac{1}{\sum_{\ell=1}^\kappa \widetilde{\gamma}_{\comps(\sigma_t, \ell)}} \nonumber \\
& = \frac{1}{|\mu|}\sum_{\kappa = 1}^{K'} \frac{\sum_{k = 1}^{\kappa} \mu_{\sigma(k)}}{\sum_{\ell = 1}^{\kappa}\widetilde{\gamma}_{\comps(\sigma_t, \ell)}}    
\end{align}
Using these expressions, we are able to calculate the overall expected waiting times in \cref{prop:waits_complete}. 
\begin{prop}\label{prop:waits_complete}
For a given admissible service menu $M$ with limiting arrival rates $\Lambda$, service rates $\mu$, and slacks $\Gamma$, let $\breve{M}$ be the residual matching and  $\{\mathbb{C}_1,\dots,\mathbb{C}_{K'}, \mathbb{C}_{K'+1}, \dots, \mathbb{C}_{K} \}$ be the collection of CRP components induced by $\breve{M}$. Then the average scaled steady-state mean waiting time in heavy traffic over all service classes $\bar{W}$ is equal to
\begin{align}
\label{eq:average_wait}
\bar{W} = \frac{1}{|\mu|}\sum_{t=1}^{T(M)} \left({\mathbb{Q}(\sigma_t) \over \mathbb{Q}(\sigma_1)+\mathbb{Q}(\sigma_2)+\cdots+\mathbb{Q}(\sigma_{T(M)})}\right)\, \sum_{\kappa = 1}^{K'} \frac{\sum_{k = 1}^{\kappa} \mu_{\sigma(k)}}{\sum_{\ell = 1}^{\kappa}\widetilde{\gamma}_{\comps(\sigma_t, \ell)}}
\end{align}
\end{prop}

Unlike in \cite{Afecheetal2019}, where the average delay depended on only the number of CRP components, we can see from \cref{eq:average_wait} that in our setting the average delay depends on both the connectivity between the CRP components, and on how the servers and service classes are allocated among the different CRP components. The connectivity between the CRP components determines the collection of topological orders $\Tcal(\Dcal, K')$. The allocations of servers and service classes among the different CRP components determines the actual values of the average delays conditional on the topological orders $\bar{w}_{\sigma_t}$, as well as the relative probabilities of observing the different topological orders.

\subsection{Menu Design}
We will now explore several design questions. While there are many ways in which the question of menu design can be approached, and many potential objectives that could be looked at, we will focus on questions regarding minimising or reducing the expected delays faced by the customers. 

The following proposition relates to the minimum possible expected delay any customer class can face.
\begin{prop}\label{prop:min_avg_waits}
Given arrival rates $\htp{\lambda}$ and service rates $\mu$ satisfying \cref{assum:heavy_traffic}, for any admissible menu $M \in \mathcal{M}(\htp{\lambda}, \mu)$,
\begin{equation*}
        \widehat{W}_{\mathbb{C}_k} \ge \frac{1}{|\Gamma|},
\end{equation*}
for all $k \in [K]$.

Furthermore, $\widehat{W}_{\mathbb{C}_k} = \frac{1}{|\Gamma|}$ for some $k \in [K]$ if and only if there exists a directed path from $\widehat{W}_{\mathbb{C}_k}$ to any other CRP component $\mathbb{C}_\kappa$ with $\kappa \in \{ [K]\setminus k\}$. This condition is trivially satisfied if there is only one CRP component. 
\end{prop}

In terms of menu design, this tells us that if the service provider wishes to minimise average delays, or the maximum expected delay any customer class faces, any menu that induces a single CRP component will achieve both of these objectives. We state this result formally in the following corollary. 
\begin{cor}
Given arrival rates $\htp{\lambda}$ and service rates $\mu$ satisfying \cref{assum:heavy_traffic}, any menu $M$ that induces a single CRP component will minimise both the average expected delays for all customer types, and the maximum expected delay faced by any customer type, across all admissible menus. The complete menu $M$, in which every customer class is served by every server, induces a single CRP component for every set of arrival rates $\htp{\lambda}$ and service rates $\mu$ satisfying \cref{assum:heavy_traffic}. 
\end{cor}
The following result is useful in designing such a menu. 
\begin{prop}
Consider a system with limiting arrival rates $\Lambda$ and service rates $\mu$. Any menu $M$ such that 
\begin{equation*}
    \sum_{j \in \mathscr{S}}\sum_{i \in [n]} \Lambda_i m_{ij} < \sum_{j \in \mathscr{S}} \mu_j, \quad \text{for all } \mathscr{S} \subsetneq [m]
\end{equation*}
will be admissible for any vector of slacks $\Gamma \in \Re^n$ such that $|\Gamma| > 0$. Furthermore, such a menu will induce a single CRP component. 
\end{prop}
This proposition tells us that we do not need to know or specify the values for the slacks $\Gamma$ to design a delay minimising menu. 

While a menu that induces a single CRP component minimises delays, it may not be desirable or even feasible to offer such a menu due to real world constraints on which servers can serve which customer types. Motivated by these sorts of constraints, we consider the question of how to design the DAG on a collection of CRP components to minimise expected delays for customers. 
\begin{prop}
Given limiting arrival rates $\Lambda$, service rates $\mu$, slacks $\Gamma$, and CRP components $\{\mathbb{C}_1,\dots,\mathbb{C}_{K'}, \mathbb{C}_{K'+1}, \dots, \mathbb{C}_{K} \}$, there will be permutation of CRP components $\sigma$ that minimises the average expected delay across all possible topological orders,
\begin{equation*}
     \bar{w}_{\sigma_t}= \sum_{\kappa = 1}^{K'} \frac{\sum_{k = 1}^{\kappa} \mu_{\sigma_t(k)}}{\sum_{\ell = 1}^{\kappa}\widetilde{\gamma}_{\comps(\sigma_t, \ell)}}
\end{equation*}
across all topological orders. The DAG or menu that will minimise delays is one that only allows for this topological order. 
\end{prop}

The slack $\widetilde{\gamma_k}$ can be either positive or negative for CRP components with a service class that is compatible server in a different CRP component. Slacks must be negative for CRP components with an empty server set, and positive for CRP components such that all service classes can only be served by servers within the CRP component. 

Thus in our example in \cref{subfig:residualmatching_b}, $\widetilde{\gamma}_4$ can be either positive or negative, as class 4 has dashed arcs representing compatibility with servers 1 and 2, while neither of these classes are within the CRP component. Since $\Lambda_3 = 0$, in order to ensure that class 3 has positive arrival rates in the pre-limit, we must have that $\widetilde{\gamma}_3 < 0$. Since $\Lambda_1 = \mu_1$, and class 1 is not compatible with any other services classes, in order to achieve stability in the pre-limit, it must be the case that $\widetilde{\gamma}_1 > 0$. Similarly, we need that $\widetilde{\gamma}_2 > 0$. 


Given that adding arcs to a DAG is achieved by adding additionally flexibility to a service system, one might think that adding an additional arc to a DAG will always reduce expected delays. However, we find that adding arcs to the DAG may potentially increase, decrease, or not effect the average delays. This can be shown through a simple two server example. This question could be of interest in a setting where a service provider is considering the benefits of cross-training servers that already have particular capabilities. This result demonstrates that the way in which flexibility is being added is important to consider, and that not every addition of flexibility will improve system performance in terms of average delays. 

==> illustrative_example.tex <==
\subsection{Illustrative Example}

To illustrate some of the concepts, let us consider the example in Figure~\ref{fig:Ex2} with four servers ($m=4$) and four customer types (i.e., $|\Theta|=4)$ which are equally distributed among the population.  

\begin{figure}[hbt]
    \begin{center}
    \includegraphics[width=9cm]{Figures/Fig_Ex2.pdf}
    \caption[Model Description]{\sf \small Example with four service classes and four servers.}
     \label{fig:Ex2}
    \end{center}
\end{figure}

The menu ${\cal M}=(n,M)$ has  four service classes ($n=4$)  and the matrices of matching $M$ and valuations $V$ are given by
\begin{equation*}
M=\left[\begin{array}{c c c c} 1 & 0 & 0 & 1 \\ 0 & 1 & 0 & 1 \\ 0 & 0 & 1 & 1 \\ 1 & 1 & 1 & 1 \end{array}\right]\quad \mbox{and}\quad V=\left[\begin{array}{c c c c} 1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \\ 0 & 0 & 1 & 0 \\ 1 & 1 & 1 & 1 \end{array}\right].
\end{equation*}
In this example, customer types $\theta=1,2,3$ have a most preferred server while type $\theta=4$ is indifferent among the  servers.

In equilibrium we expect that each customer type will select the service class  that maximizes the likelihood of being served by the most preferred server, that is type $\theta$ selects service class $i=\theta$ for $\theta=1,2,3$ while type $\theta=4$ is completely indifferent. In this case, let us guess an equilibrium with $\lambda_i= \Lambda\, \rho/4$. Solving for the resulting matching probability\footnote{Note that the QP does not provide optimal flows in this example.} we get
$$p={1 \over 16}\left[\begin{array}{c c c c} 11 & 0 & 0 & 5 \\ 0 & 11 & 0 & 5 \\ 0 & 0 & 11 & 5 \\ 5 & 5 & 5 & 1 \end{array}\right].$$
Also one can show that in the limit as $\rho \uparrow 1$ we have
$$\lim_{\rho \uparrow 1} (1-\rho)\,W_i = {1 \over 4} \qquad i=1,\dots,4.$$

Hence, it follows that $\lambda=(1,1,1,1)$ is an equilibrium in heavy traffic that produces a vector of utilities (assume $\delta=1$)
$$U^*={1 \over 16}\,(7,7,7,12).$$




Can we find a different menu ${\cal M}$ that would generate a higher vector of utility in equilibrium?


\begin{figure}[hbt]
    \begin{center}
    \includegraphics[width=9cm]{Figures/Fig_Ex2b.pdf}
    \caption[Model Description]{\sf \small Example with four service classes and four servers.}
     \label{fig:Ex3}
    \end{center}
\end{figure}
